Filaments of The Slime Mold Cosmic Web And How They Affect Galaxy Evolution

We present a novel method for identifying cosmic web filaments using the IllustrisTNG (TNG100) cosmological simulations and investigate the impact of filaments on galaxies. We compare the use of cosmic density field estimates from the Delaunay Tessellation Field Estimator (DTFE) and the Monte Carlo Physarum Machine (MCPM), which is inspired by the slime mold organism, in the DisPerSE structure identification framework. The MCPM-based reconstruction identifies filaments with higher fidelity, finding more low-prominence/diffuse filaments and better tracing the true underlying matter distribution than the DTFE-based reconstruction. Using our new filament catalogs, we find that most galaxies are located within 1.5-2.5 Mpc of a filamentary spine, with little change in the median specific star formation rate and the median galactic gas fraction with distance to the nearest filament. Instead, we introduce the filament line density, Sigma_fil(MCPM), as the total MCPM overdensity per unit length of a local filament segment, and find that this parameter is a superior predictor of galactic gas supply and quenching. Our results indicate that most galaxies are quenched and gas-poor near high-line density filaments at z<=1. At z=0, quenching in log(M*/Msun)>10.5 galaxies is mainly driven by mass, while lower-mass galaxies are significantly affected by the filament line density. In high-line density filaments, satellites are strongly quenched, whereas centrals have reduced star formation, but not gas fraction, at z<=0.5. We discuss the prospect of applying our new filament identification method to galaxy surveys with SDSS, DESI, Subaru PFS, etc. to elucidate the effect of large-scale structure on galaxy formation.

==> refereereport.tex <==
We are grateful to the anonymous referee for their detailed consideration of this manuscript and their detailed comments and suggestions to improve it. We have addressed these comments below, and prepared a revised version that we believe will assuage the referee's doubts and concerns. We present our responses to each of the concerns raised in the report below.
----

REFEREE REPORT

I have read with interest the paper entitled ‘Filaments of the slime cold cosmic web and how they affect galaxy evolution’ by Hasan et al.. This paper uses a novel density field estimator as the basis for the identification of filamentary structures. It presents some comparisons with the more widely used Delaunay Tessellation Field Estimator. The idea of the paper is extremely interesting, since we know that DFTE is very sensitive to the effects of noise compared to other estimators (Busch and White 2020). The paper also aims at performing an interesting and long-needed analysis of how filaments shape the properties of galaxies by investigating relations between some filament properties, SFR, and gas fractions.

However, I have significant major concerns regarding the methods and results of the paper, which make me seriously doubt about the robustness of the claims made by the authors. These are presented in the following, without any particular other.

Major concerns:


1. There is a serious problem regarding the physical scales of the different filamentary structures. The cosmic web is intrinsically multi-scale, and filamentary structures can be found from molecular clouds at pc scales, to the large Mpc-scale structure of the web, including the kpc-scale filaments feeding galaxies with cold gas. While all filamentary, these structures are very different in their physics and properties. This paper seems to mix kpc- and Mpc- scales without any mention or discussion. For example, an obvious alarming result is the fact that the authors find that all the considered galaxies are in filaments, which is in clear contradiction with all the literature in the cosmic web field. This is also in contradiction with their own study, given that they calibrate the filament end-points to match massive nodes (hosts of galaxy clusters, i.e. at the largest-scales of the web), but the resulting MCPM filaments are a clear mix between small- and large-scale filaments (one can clearly see this in their Fig. 4). The authors should carefully revise their filament catalogues and physical calibration and address in length the validation and purity of their filament catalogues. I have made more specific comments below.


----

RESPONSE:

We thank the referee for raising this very important point about our paper. We address each of the referee's specific comments below, and have made many changes throughout this paper.  In short, we are focusing on Mpc-scale and larger filaments and therefore probing large-scale structure. We show this using filament length distributions too. We postulate that some of the referee’s specific concerns about the apparent sizes of filaments being small could be due to projection effects of individual filament segments in finite 2D slices. 

We hope our corrections or additions below will help ease the referee’s concerns.
----


2. Another important problem is the fact that the authors do NOT disentangle the effects of cosmic nodes in their analysis of galaxy properties. Is it well established that nodes host redder galaxies with respect to other cosmic environments, but in the current version of the paper this is completely dismissed. Please take into account the effect of nodes by removing/masking the galaxies belonging to r200 (or 3xr200) of massive galaxy clusters and performing your analysis on the remaining galaxies. Given the current state of the paper, I am not convinced by the any of the trends attributed to filaments.


----

RESPONSE:

The referee is absolutely correct that cosmic nodes and/or massive halos can contribute significantly to the filament-galaxy connection (as we have shown in Paper I as well). We introduce a new subsection (3.3: “Accounting for massive halos”) where, as per the referee’s suggestion, we remove the galaxies within 3R_200,c of the 0.5% most massive halos at each redshift. Despite small reductions in the trends, most of our qualitative conclusions — especially the general drop in gas fraction and star formation in high line-density filaments at low-z — hold. Therefore, we are confident our results are not simply due to the hydrodynamical effects of massive halos/nodes, but that they are likely due to filaments themselves.
----


3. I have several major concerns regarding the comparison between the filament catalogues coming from the two different methods, MCPM and DTFE densities. I have made several detailed comments below. This is a key point of the paper that deserves to be carefully addressed.


----

RESPONSE:

We thank the referee for their rigorous assessment of our filament catalogs and methods of constructing them. We address all of the comments pertaining to this issue below, and are hopeful that the referee’s major concerns will be alleviated.  
----


4. I have been very uncomfortable with the many bold claims made by the authors, which are either an over-interpretation of results or based on shortcuts and wrong assumptions. Throughout the paper I have found a large number of inaccuracies and misunderstandings that are pointed out in the line-by-line analysis below.


----

RESPONSE:

We are grateful to the referee for pointing out these shortcomings. We address these concerns individually below, as well as make necessary changes in the revised manuscript.
----


6. The paper is extremely long and suffers from many repetitions, cross-references to different sections, and back-and-forwards. I strongly encourage the authors to revise the text, re-organise it to make it more concise and avoid repetitions. This would definitely give more impact to the main results of the paper, without the need of the strong and inaccurate claims. I believe that the length of the paper can be reduced by at least 1/3 without any loss of information.


----

RESPONSE:

We do agree with the referee that the paper is somewhat long, but after careful consideration, we believe its length is warranted to adequately and accurately describe our results, as well as address all of the referee’s concerns. We made an honest effort in improving the structure of this paper, and have significantly re-structured a lot of the text. We believe there are far fewer repetitions, cross-references, etc. 
----

My more detailed comments are stated below:

Abstract:

‘A novel method for identifying cosmic web filaments’. What is novel and interesting is the density estimator. Technically speaking, the method for identifying filaments in this paper is the one of Disperse, i.e. based on the topology of the density field computed by Morse theory, therefore not new. Please rephrase this sentence and the modify accordingly in the relevant parts of the main text.
----

RESPONSE: We thank the referee for this suggestion, and have edited our abstract to address this suggestion.
----

Introduction:

I found the introduction well-written and structured. It was pleasant to read. My main concern is that an introduction on the multi-scale nature of filaments in lacking. I suggest to add such discussion and to specify clearly which scales are the authors focusing on in the paper.
----

RESPONSE: We thank the referee for this important suggestion. We have added many lines of text in the introduction (L. 67-85) discussing the multi-scale nature of filaments and specifying that focus on the large-scale (Mpc or higher).
----

L. 78-101: The authors should also consider filament finders that appeared after 2028, such as T-rex (Bonnaire+2020), 1-DREAM (Awad+2023), and others.
----

RESPONSE: We thank the referee for bringing these works to our attention. The references have been added.
----

L. 141-143: There might be a typo In this sentence?
----

RESPONSE: Indeed there was a typo, which we have now fixed.
----

L. 166: DFTE provides a *continuous* density field by linear interpolation (this is even mentioned this further down in the text). Please be more precise here.
----

RESPONSE: We have revised this statement, and elsewhere in the text where something similar appears.
----

L. 183: ‘method’ —> ‘density field reconstruction’
----

RESPONSE: We have corrected this.
----

Section 2.1

L. 216: ‘we’ —> ‘the authors of that paper’? I suppose you are using public data from the TNG group and subgroup catalogues, or did you run the FoF and SUBFIND algorithms yourself onto particle data?
----

RESPONSE: We have updated the text to clarify that this was already done, and we merely obtained these catalogs from the online repository
----

Section 2.2

L. 256: ‘Apply the 3D density field estimate to mse’ —> ‘Apply mse to the 3D density field estimate’ ?
----

RESPONSE: No, we apply as input the grid that represents the 3D density field — in the ND network format enabled by DisPerSE– to mse, which in turns computes the Morse Smale complex from this grid. (Note: This is the traditional application of mse (i.e., with the DTFE implementation), but later, when using the MCPM density field, we use a ND field file format as an input to mse. This is mentioned in the text too.
----

L. 277: ‘two nearest neighbors’: are you smoothing the density field twice? Please be more explicit in this smoothing procedure of the input *density field* that is known to have important effects on the resulting skeleton (Malavasi+ 2022, Galárraga-Espinosa+2023b).
----

RESPONSE:

As in Malavasi+22, we smooth the density field value at the position of each galaxy by averaging it with the density field for all galaxies that share an edge of the tetrahedrons of the tessellation with this galaxy. 
----

Section 2.3

L. 360: It is not clear to me what ‘time-averaged equilibrium density field’ means in this context. Where does the time component come from? Please rephrase or be more explicit for clarity.
----

RESPONSE:

We thank the referee for asking us to clarify this point. MCPM is run by agents navigating towards and making connections through the data, and this happens across many timesteps, with the agents moving at each timestep. Eventually — usually about hundreds of timesteps later — the fit has “converged”; in other words, the fitness function converges and there is no significant change in the density of the agents afterwards if the hyperparameters are not changed. The equilibrium density field is the trace density field averaged over all the timesteps or iterations. 

We have updated the text to reflect this clarification. 
----

L. 376: “In Section 2.4, we compare the mapping between the [...]”I strongly encourage the authors to present such analysis here. This Section seems to be the optimal place to present the aforementioned mapping and some visualisations of slices of the MCPM density field vs the underlying DM density field. Doing so would avoid many repetitions, thus increasing the clarity and conciseness of the paper.
----

RESPONSE:

We are grateful to the referee for this very important recommendation. We have added a new subsection in the text (2.3.2: “Comparing Density Fields”) to rigorously compare the mapping between the MCPM and DM density fields. Furthermore, as per the referee’s additional suggestions below, this is also where we compare the mapping between the DTFE and DM density fields.
----

L. 386-388: Even if the details are presented in Elek+2022, I suggest the authors to include a sentence or two with more information regarding the fitness function, which seems to be crucial for the extraction of the density field. This will also help in the discussion in L. 413.
----

RESPONSE:

We have added some text to elucidate the fitness function further. Mathematically, this function is a maximum likelihood estimator of the trace density field normalized by each data point’s mass. It ensures that the data points are almost all reliably included in the fit and the mass of a galaxy influences the strength of the connections in the density field. We also discuss caveats to this function.
----

L. 407-408: This sentence seems to be in contradiction with the text in lines 371-376. Please rephrase or comment to be consistent.
----

RESPONSE:

We have restructured this portion of the text and removed this sentence entirely in the revised version. Instead, we have added two new subsections where we explain in detail how we correlate the MCPM and DM density field in TNG100 specifically. 
----

L. 397-415: Is the sharpness the only parameter of the code? I strongly encourage the authors to provide some visualisations of the reconstructed density field with different sharpness parameters (see my comment above).
----

RESPONSE:

We thank the referee for raising this point and making this suggestion. In short, no, there are a few other hyperparameters that may also be important. We have added a new subsection (2.3.1: “Calibrating Input Parameters”) where we lay out the details of the hyperparameters and our entire methodology of calibrating them such that the output density field provides the best mapping against the DM density field. In Table 1, we list the parameters we deem optimal at each redshift and in Appendix A, we present additional visualizations of the density field generated with different hyperparameters.
----

L. 425-426: ‘previous studies’ —> please provide references. Also, this last sentence is incorrect for reconstructions with the Delaunay tessellation. Please specify clearly if you are referring only to the MCPM method.
----

RESPONSE:

Here we were referring to MCPM specifically. In any case, we have removed this sentence and in the revised version clarified the results pertaining to this statement from previous studies.
----

Section 2.4
> In this section, it should be stated more clearly that Disperse is applied in different ways to the MCPM and Delaunay density fields. In one case Disperse is applied to a grid, while in the other, to point-data. This difference is fundamental. My suspicion is that many results of the paper arise solely from this technical aspect, regardless of the density reconstruction.

> A fair comparison between the filaments extracted from the two different density estimators would result from projecting the Delaunay density field into the same 512^3 grid as the one used from MCPM, and running Disperse on this grid, using the cut parameter. This is one of my major concerns of the paper.

----

RESPONSE:

We thank the referee for raising this major concern and we have attempted to address this is a clear and methodical way. The new section 2.3.2 presents detailed comparisons of the MCPM, DM, and DTFE density fields, including visual and statistal tests to illustrate how well they compare with each other. We have computed continuous DTFE density fields grids using the publicly available DTFE package (Cautun+19) and compared them on different smoothing scales. We illustrate in Figure 2 that (1) MCPM is visually a much better match to the DM density field than the DTFE density field on the same smoothing scale, and (2) the MCPM overdensity correlates far better with DM overdensity, with lower RMSE score, higher Pearson r-value, much less scatter, and a much more monotonic mapping, than the DTFE overdensity. We find similar results from our comparisons at higher redshifts too. 

We attempted to follow the referee’s suggestion and run DisPerSE on the DTFE density field projected on to the same grid as that of MCPM. Unfortunately, the resulting structures did not appear to look like filaments for any of the tens of persistence cut values we tried. A comparison of the “filamentary stucture” from the DTFE grid and MCPM can be seen in additional Figure A2, where we see that from these DTFE grids, the filaments appear to be looped structures and not resembling filaments as we expect them at all. No smoothing levels or resolution scales solved this problem — unphysical strcutures were identified as filaments in each case. Since the objective of our paper is to identify filaments from MCPM density fields, we consider it beyond the scope of our work to extract real physical filamentary structure from the DTFE grids. Therefore, we continue with our analysis of MCPM-based filaments from a grid with DTFE-based filaments from the discrete network. 
----

L. 433: Does 1e8 come from the 512^3 grid? Please specify for clarity.
----

RESPONSE:

This is correct. We have updated the text.
----

The first paragraph of the section would be more impactful if the authors explicitly show examples of the MCPM density field in a 2D slice, and compare them to the corresponding Delaunay density field **projected into the same 512^3 grid**.
----

RESPONSE:

We have presented such a visual comparison in Figure 2.
----

L. 453: Why is this downsampling needed? Please say it in the text.
----

RESPONSE:

We explain our process of post-processing the density fields via downsampling and smoothing in sections 2.3.1 and 2.3.2. There, we explain our rationale for the downsampling and smoothing. Briefly, we find that the higher the downsampling, the better the correlation between MCPM (or DTFE) and underlying DM density field (which is a desirable outcome as we would like to best approximate the true matter distribution to obtain the most accurate description of large-scale filaments). However, too much smoothing would blur out some of the finer structures of the cosmic web. As a compromise, we choose a voxel resolution scale of 256^3, corresponding to about ~0.5 Mpc, which would resolve filaments down to about 1 Mpc in scale (with >2 resolution elements), as is our focus in this work. Using a non-downsampled 512^3 grid gives much higher stochastic noise in the density field and results in a signficantly worse correlation with DM density than any of the downsampled grids. 
----

Regarding the matching of CPmax with massive haloes.


- For the dark blue and red histograms of Fig.2, why are you considering 1 Mpc instead

of R200? In the text you say this is ‘to account for the smoothing of the filamentary skeleton’, but this smoothing does not change the positons of the CPmax, as you clearly stated somewhere else in the paper.
----

RESPONSE:

The referee is correct in raising this concern and we admit this was an erroneous statement. In our new figure concerning the matching of CPmax with massive haloes (Fig 3), we choose 1 Mpc as the separation between CPmax and log(Mh)>11 halos as this corresponds to about twice the smoothing scale (~0.5 Mpc). Therefore, this would account for the smoothing of features on small scales in post-processing of the density fields. We have updated the text in the appropriate place.
----


- Also, it is not obvious to me that maximising the number of filaments should be considered as a criterion for calibrating the skeletons, since shot noise can also lead to the identification of filaments. This particularly the case for the identification of filaments from the MCPM density field, where a wide range of scales seem to be mixed (from small-scale filaments to the cosmic large-scale ones). In other words, how can you be sure that the ~30 000 filaments you identify in this case (I am reading Fig. 2, cut= 1000) are all physical structures and not noise-induced? Please address this point in the main text.


----

RESPONSE:

The referee is absolutely correct in pointing out this important flaw in our methodology and assumptions about the purity and completeness of our filament catalogs. In the revised paper, we have removed any requirement that the number of filaments be maximized in any of the reconstructions. As for the physical scales of the filaments, we address this comment below.
----

I strongly encourage the authors to add a proper quantitative comparison of the final Disperse filaments from both the MCPM and Delaunay cases. This is needed to support the conclusions written in the main text. This comparison should include:


1. The input density distributions (probably rescaled by some quantity to ease the

	comparison), to prove that MCPM probes wider density ranges, including lower

	density values that escape to the Delaunay reconstruction.


2. The filament length distributions from both MCPM and Delaunay cases, in order to

	show the different scales present in the filament catalogues.
----

RESPONSE:

We are grateful for the referee’s suggestions here. We believe we have addressed these comments adequately, by means of detailed discussion as well as additional figures. In particular, we point the referee to (1) Figure 2, which contain both visual and statistical comparisons of the density distributions between MCPM and DTFE, and (2) Figure 3, which contain the filament length distributions for different persistence cuts in the DTFE and MCPM filament catalogs at z=0. In addition, please take a look at our new Figure 6, which show the length distributions for our chosen optimum persistence cuts at different redshifts. We are confident that these figures, and all the accompanying texts establish that MCPM filaments are probing large sacle strcutures on the order of Mpc or larger, with only a small fraction (<10%) being below 1 Mpc. The DTFE filaments are actually much smaller on average than the MCPM filaments and a larger fraction (~25-30%) are <1 Mpc in total length.
----

L. 519: ‘a non-DTFE (MCPM) density field’ —> ‘a grid’.
----

RESPONSE:

We have updated the text such that we no longer say 'non-DTFE (MCPM) density field’.
----

L. 527-530: I am puzzled by this result. A higher persistence ratio should result in a decrease of the number of identified peaks (or CPmax), so the fraction of matched halos should decrease (because the number of haloes is of course unchanged). Please comment.
----

RESPONSE:

The light blue bars in our new Fig. 3 represent the fraction of log(Mh)>11 halos that are within 1 Mpc of a CP_max. Thus, the fraction is Num(halos)/Num(CP_max), and the denominator of this fraction decreases with increasing persistence, not the numerator (as we believe the referee was implying). On the flipside, the orange bars indicate the fraction of CP_max within the virial radii of very massive halos. Here, the fraction is Num(CP_max)/Num(halos), so the numerator goes down with increasing persistence and consequently, this fraction decreases with large-enough persistence.

Furthermore, we no longer look at CPmax ≤ 1 Mpc of log(Mh) ≥ 12 halos (in the previous version, the dark blue bars).
----

L. 546: see my comment above regarding the maximisation of the number of filaments.
----

RESPONSE:

Please see our response to that comment above. Number of filaments is no longer considered in our analysis here.
----

L. 582-590: I remind the authors that the skelconv function of Disperse smooths the positions of the filaments, and it is usually applied for cosmetic reasons to soften the angles between filament segments. This function does NOT change or smooth the density field. I believe that here you are referring to a different type of smoothing as the one in Galarraga-Espinosa+ 2023. In that paper, the authors refer to the smoothing applied to the density field (using the **netconv** function, prior to mse). Please correct this part of the text.

Given that it is mentioned by the authors, I strongly encourage them to present a justification of the smoothing (if any) of the MCPM density field using the netconv function.
----

RESPONSE:

We thank the referee for catching these erroneous statements and remove them. We have modified the paragraph in question to refer to smoothing of the filaments segments. We also separately discuss the smoothing of the MCPM density field in detail in section 2.3, as mentioned above.
----

L. 594: This should appear before in the text, to help the reader know which filament scales you are probing. Also, if a filament segment is at most 1 Mpc in length, this means that most of the filament segments link **at most** 2 voxels of effective size 0.5 Mpc. Is this correct?
----

RESPONSE:

Yes, this is correct. And we do in fact include this information in the text beforehand, as mentioned above.
----

Section 2.5

L. 607: Figure 3 is nice. Please include include a visualisation of the underlying MCPM and Delaunay densities projected onto the same grid (if not done before), and overlap DTFE filaments from both point-like and grid runs. Otherwise, I am not sure that what we see in Figure 3 is a fair comparison between the 2 different types of density fields (which I believe, is the message the authors aim at conveying).
----

RESPONSE:

We have presented such a visual comparison between the different density fields in Figure 2 and a comparison between the identified filaments from each case in Figure 4. Once again, we mention that we attempted to carry out the cosmic web reconstruction using DTFE grids instead of discrete point inputs, and obtained unphysical filamentary structure (see our response above). We again ask the referee to look at our additional Figure A2 for proof that this does not produce reasonable filamentary structure.
----

L. 613: What is the persistence value of a filament? Please clearly define this quantity in the main text.
----

RESPONSE:

We neglected to specify this in the previous version of the text. The persistence value we present in the new Figure 3 is the mean persistence value of the two critical points at the extremities of each filament segment. We have defined and elucidated this in the text.
----

L. 621: Same comment as above regarding the number of filaments.
----

RESPONSE:

Please see our response to those comments above.
----

L. 622: Why should most of the galaxies be connected? This is worrying because all galaxies should NOT be in filaments. According to Cautun+ 2014, and Ganeshaiah- Veena+2019 about 50% of galaxies belong to filaments, the remaining ones being in one of the other cosmic structures (walls, voids, or nodes). Please justify your motivations for this strong physical prior and discuss the scales of the filaments you are probing.
----

RESPONSE:

We believe this is a result of our inability to properly communicate our results and our justifications. First of all, we have removed the figure and discussion surrounding galaxies being connected to filaments. Our main reasoning behind considering thsi physical prior is that galaxies and their parent halos represent peaks of the matter density field and therefore filaments should more-or-less be tracing them. 

Importantly, we point out that our results are NOT in contradiction to those of, e.g., Cautun+14, and Ganeshaiah-Veena+19, for several reasons. Different studies use different methods to identify filaments which results in different classification results for cosmic web structures (as shown in Libeskind+18 and others). Different works also classify galaxies/halos as “belonging” to different environments such as filaments, walls, and nodes. This is something that is very method-dependent and is something that we do not attempt at all. We do not assign galaxies to filaments or other particular web environments. DisPerSE gives the discrete locations of critical points that are linked together to form 1D filament line segments and we therefore consider galaxies with respect to 1D spines of filaments. Many of the galaxies that reside close to filament spines are could very well be physically associated with nodes or walls, but again this is not something we tackle in this work.

We have added discussion of this in section 3.1.1 (L. 1155-1179). 
----

L. 626: Please remove this parenthesis. You have shown above that this cut is supposed to be the best, so it is surprising to call it ‘relatively generous’.
----

RESPONSE:

The referee is correct and we have removed this text.
----

L. 628-631: Please remove or correct this sentence after performing the study of filaments extracted from the Delaunay density projected on the same grid as the MCPM one.
----

RESPONSE:

This result holds in the revised version of the paper. 
----

L. 636-641: Given all my comments above, I am not sure I agree with this sentence. I would like the authors to provide clear proof that the ~30 000 filaments detected in the MCPM case are physical structures, or to soften this sentence. The part ‘filaments that should nevertheless connect galaxies based on visual inspection’ is extremely weak and naive (e.g. in a 2D slice, walls are projected as filaments, so not all the observed filamentary structures are actual filaments in 2D...). In line with my comment above, it is worrying for me that the authors expect all the galaxies to be connected by filaments.
----

RESPONSE:

We agree that this statement was perhaps a little too strong. However, having repeated our analysis as per the referee’s multiple suggestions, we we arrive at a similar conclusion that identificaction of large-scale filamentary structure is actually improved significantly by using MCPM instead of DTFE. 

We have removed the statement ‘filaments that should nevertheless connect galaxies based on visual inspection’ and instead point the referee to our response above regarding galaxies in filaments as well as the text in 3.1.1 (L. 1155-1179).
----

L. 655: Please define clearly in the text what you mean by ‘les prominent filaments’. This is a term that appears multiple times in the text without being explicitly defined. Are these small-scale filaments such as those in Ramsoy+ 2021? Or are these long and large-scale cosmic filaments such as those of Gallaraga-Espinosa+ 2020? This should be addressed in a dedicated discussion regarding filament scales.
----

RESPONSE:

We thank the referee for bringing this shortcoming to our attention. First of all, we have defined the average persistence of filament segments in the first paragraph of section 2.5. Second, we explain less persistent/prominent filaments in the next paragraph more clearly (in terms of the robustness of identified filamentary structure). Third, we bring the definition of local filament line density, sigma_fil, to section 2.5 to show that this quantity for a segment is directly proportional to average persistence of the segment. Figure 5 shows this correlation, and exemplifies that less prominent filament segments are in fact low in sigma_fil. 

Finally, with regards to filament scales, we once again point the referee to the L_fil distributions (Fig 3 and 6) to show that we are probing large-scale filaments with MCPM. We have also added a paragraph discussing filament scales in the discussion section 4.2.1 (L. 1795-1813).
----

Figure 4: These visualisations are a clear example that the MCPM filaments mix large- and small- scale filaments. It is crucial to tackle this aspect given that different scales are not ruled by the same physics, thus resulting on very different filament properties accross scales.
----

RESPONSE:

We believe the 2D projection effect possibly contributed to the referee’s belief in some of these filaments are small-scale. Specifically, the filaments appearing so small are due to projection of filament segments in finite 2D slices. We show in the plot only filament segments, so the entire filamentary structure may not be captured within this 10 Mpc thick slice. Additionally, our L_fil distributions clearly show that MCPM filaments are in almost all cases large-scale structures (see many of the responses above). Finally, we remind the referee about the scales of the visualization — each minor tick on the x- and y-axis corresponds to 5 Mpc, which is by no means a small physical scale.
----

L. 685-689: Same comment as before regarding connection of filaments to galaxies and Disperse applications to grids vs point-like data.
----

RESPONSE:

Please see our repsonses above.
----

L. 702-709: I am not convinced by this argumentation, 0.2 Mpc is not very far from 0.1 Mpc. Moreover, given the grid size, 0.2 Mpc corresponds to filaments occupying only 1 voxel! These are definitely below the resolution level and should be considered as spurious filaments. This comparison should be performed with filaments from a Delaunay density projected on a grid. Please remove the last sentence of the paragraph, this is clearly too strong given the results you show.
----

RESPONSE:

We concur with the referee’s doubts and have re-done this analysis and removed this argument.
----

L. 710-719: Please motivate in the text why you correlate persistence with the DM density field. Please include the same study using information from Delaunay densities projected into the same grid. Also, I suggest to move this study to an earlier section in the paper.
----

RESPONSE:

We agree fully with the referee’s suggestion here and show the mapping between DM and MCPM (and DTFE) density fields to section 2.3. We also remove the correlation between the DM density and persistence, as we believe it does not add to the arguments we are trying to make in this study.
----

Section 3.1.1

Fig. 7: it seems to me that the d_fil bins are different for the DTFE and MCPM cases? If this is the case, please perform the comparison using the same binning.
----

RESPONSE:

In the text, we explain how we binned the d_fil in each case. We bin the d_fil such that there is essentially an equal number of galaxies in each bin, in order to maximize the statistical signal of each bin. We refer the referee to Figure 8 (d_fil CDFs) to illustrate the point that there are very different fractions of galaxies for a given d_fil between the MCPM and DTFE cases. Thus, performing the comparison with the same bins will result in very few (if any) galaxies in the low d_fil bins for DTFE and high d_fil bins for MCPM, weakening the statistical conclusions we can draw from this figure.
----

L. 786-788: Please remove the italics. As the authors state later on in the paper, this is due to the large number of filaments in the MCPM case. I am still not convinced that all of them correspond to physical cosmic (large-scale) filaments, in which case this sentence is irrelevant.
----

RESPONSE:

We sincerely hope that the referee is more confident in our filament catalogs probing large-scale filaments after the myriad corrections and additions we have made in section 2. Regardless, we have removed most of the italicization of this sentence and in the revised version have only italicized the term “no effect”. 
----

L. 790-792: This result at high z is new and interesting. Can the authors comment on what would explain this? I believe this is not explicitly mentioned at any point in the long discussion section.
----

RESPONSE:

Indeed this is a highly interesting result of our work. We have discussed it at several points in the Discussion, which the referee may have missed. Specifically, we point the referee towards section 4.2.1 and 4.2.2 for detailed discussion of this phenomenon.
----

L. 805-806: Again, this is a shocking statement to me that hints that there is a problem in the filament catalogue (seedy many comments above).
----

RESPONSE:

Once again, there may be a strong disconnect with what we are trying to communicate and the referee’s perception thereof. We have corrected this statement to say, ”virtually all galaxies live close to a filament spine” instead. This is a better characterization of our results and it does not claim that all galaxies are located IN filaments, rather close to fiament spines.

As in our response to a point above, we point out that our results are NOT in contradiction to those of, e.g., Cautun+14, and Ganeshaiah-Veena+19, for several reasons. Different studies use different methods to identify filaments which results in different classification results for cosmic web structures (as shown in Libeskind+18 and others). Different works also classify galaxies/halos as “belonging” to different environments such as filaments, walls, and nodes. This is something that is very method-dependent and is something that we do not attempt at all. We do not assign galaxies to filaments or other particular web environments. DisPerSE gives the discrete locations of critical points that are linked together to form 1D filament line segments and we therefore consider galaxies with respect to 1D spines of filaments. Many of the galaxies that reside close to filament spines are could very well be physically associated with nodes or walls, but again this is not something we tackle in this work.

Please see the discussion of this in section 3.1.1 (L. 1155-1179). 
----

L. 812-835: Important point. It is not transparent given the curent version of the paper why the authors imply a relation between filament widths and line density. Is the latter the density perpendicular to the filament, or along the spine of the filament? This is not clear from the definition in Eq. 1 and the text. Does the sentence ‘the sum of the MCPM over density in a filament segment’ mean that you consider the grid voxels belonging to the spine of the filament? Also, given Eq. 1, I don’t understand why you call this Sigma_gils instead of Sigma_seg (given that you are dividing by the length of ONE segment).
----

RESPONSE:

We thank the referee for raising a very important point which caused us to refine our language and be a lot more precise in what we are trying to convey. We have defined sigma_fil earlier, in section 2.5. It is the local filament line density, i.e., MCPM overdensity summed along a filament segment. So, it only considers grid voxels belonging to the spine of the filament. We believe changing the naming of this quantity to something like sigma_seg may be confusing to those unfamiliar with the DisPerSE nomenclature of segments. As we clarify in section 2.5 (L. 955-966), this is a measure of the local 1D line density of filament segments.
----

What do you mean by ‘global line density’ in line 829. This paragraph needs to be more explicit to gain in clarity.
----

RESPONSE:

We also address this point in the aforementioned portion of the text. The line density for an entire filament is the density along ALL line segments making up a filament. Some filaments can be >50-100 Mpc long, and with significant variations in matter density (gas, DM, stars, etc.) along different segments of those filaments. We wanted to isolate the effect of the nearest filament segment instead.
----

L. 850-866: Important point. What do you mean by the ‘prominence of a filament’? The authors seem to be implying that persistence can be a proxy for filament thickness, but this is not correct. Persistence is a measure of the robustness of a filament with respect to the noise. Please explicitly prove your implications in the text, or correct this paragraph and the analysis deriving from it.
----

RESPONSE:

We thank the referee for bringing this shortcoming to our attention. First and foremost, we have removed all implications of filament “thickness” in our work, including in figures. We characterize quantities in terms of high or low line density, and recognize that this is not necessarily related in a 1:1 way with the physical thickness of filaments. We also show in section 2.5 that the filament line density for a segment is directly proportional to average persistence of the segment, i.e., less prominent filament segments are in fact low in sigma_fil (see Figure 5)
----

L. 868: For this comparison, did you project the density field into the same grid and summed all the voxels along filament segments as for the MCPM case? Anything different from this would not be a fair comparison.
----

RESPONSE:

We remove this comparison entirely from our revised paper.
----

Fig. 9: Please include a presentation of the different panels in the caption of the figure.
----

RESPONSE:

We have added this in the caption of the new version of this Figure (Fig 5).
----

L. 878-883: This ‘further investigation’ is simply an effect of your method. Please revise this discussion (and place it in an earlier section of the paper) after addressing my comments regarding grids.
----

RESPONSE:

We have removed this analysis; this discussion is no longer relevant to our work.
----

L. 893: ‘A less complete filament identification’: Is it? Or is it just an identification of the *large-scale* filaments. This goes with my comments above regarding the scales and purity of the MCPM filaments.
----

RESPONSE:

Please see our many detailed responses to several comments above and analysis and results presented in the text.
----

L. 897-901: see my comment above regarding persistence as a proxy for width. I do not believe this is can be considered an acceptable justification.
----

RESPONSE:

Please see our response to the comment above.
----

L. 917: Please state in the text the approximate widths in Mpc of ‘thick’ and ‘thin’ filaments, so the reader can understand what scales you are aiming at probing. Regardless, I would be more comfortable by replacing ‘thick/thin’ by ‘low/high Sigma_fil’ here and throughout the text. Are thick filaments large-scale (Mpc) filaments and thin ones kpc-scale?
----

RESPONSE:

We thank the referee for bringing this shortcoming to our attention. Again, we have removed all implications of filament “thickness” in our work, including in figures. We characterize quantities in terms of high or low line density, and recognize that this is not necessarily related monotonically with the filament thickness. We also discuss approaches used by other studies to quantify filament widths, which is not what we aim to characterize here. Our filaments are large-scale, and they do not separate by filament thickness, line density, or other similar measures.
----

Fig. 11: Please state explicitly which cut in d_fil you chose.
----

RESPONSE:

We do not choose a d_fil cut for this figure. As we mention in the text, there are are no changes in our results when we restrict our galaxies to d_fil = 1 or 2 Mpc.
----

Section 3.1.2

For completeness and fair comparison, I strongly suggest the authors to include an analysis of how SFR correlates with 1+delta(DM). This will allow to probe the specific impact of filamentary structures beyond local overdensity. There was an attempt to do so in the discussion section, but I believe the method adopted by the authors gives inconclusive results (see my comment below).
----

RESPONSE:

We thank the referee for making this suggestion. We present a complementary analysis of the effect of quenching/redness on mass and local MCPM overdensity. Since we already showed a good mapping between MCPM and DM overdensity, we believe this equivalently accounts for the local overdensity effect. The resulting Figures 10 and 11 give similar results, albeit some differences for the satelllites (right panels).
----

L. 1028: the ‘highest’ line density filaments quoted here corresponds to a log value of 2. This is clearly not one of the highest values in Fig. 12. Please correct or rephrase.
----

RESPONSE:

The referee is correct in pointing out this error. We have corrected this in the text, where the number is now, correctly, 10^8 Mpc^-1.
----

L. 1052: The ‘very low Sigma field’ corresponds to logSigma=6. These values are in contraction with what you say in l. 1028. Please be consistent.
----

RESPONSE:

We have corrected this contradiction in the text.
----

Section 3.2

Given the aims of this section and the relation that is built with SFR, the authors should consider the fraction of **cold and dense** gas instead of the fraction of all gas. Indeed, hot gas (>1e7K) or WHIM gas in filaments should be excluded from this study. Please do so and update the corresponding plots and discussion.

Moreover, this section presents many strong claims that need to be justified by exploring all the other factors and physical mechanisms that could be responsible for SFR quenching (presence of AGN, local density, connection to cold flows, gas recycling in the CGM, etc). This is obviously not the aim of the paper, so I ask the authors to tone down their interpretations.
----

RESPONSE:

We thank the referee for making these two very important and related points. However, isolating the cold and dense gas in each galaxy and repeating our measurements is very involved and well beyond the scope of this paper. Indeed there are many additional factors such as AGN feedback, gas recycling, etc. that need to be considered to identify the true physical connections at play here. We are planning a follow-up paper which addresses all of these very important issues in the detail they deserve. In this follow-up, we will quantify the fraction of cold and dense gas as the referee suggested, as well as the effect of mechanisms such as AGN feedback. We have toned down our interpretations as well, and added text in section 3.2 to make clarifications.
----

L. 1096: “difficult to explain” —> please remove the contribution of massive haloes in your analysis.`
----

RESPONSE:

We have decided to remove the f_gas vs d_fil analysis for the sake of brevity and since it does not seem to add much to our paper. We already established a lack of correlation between quenching and d_fil for MCPM filaments and the existence of a correlation between quenching and sigma_fil, so we proceed directly to measuring the correlation between f_gas and sigma_fil.
----

L.1103-1106: This is clearly an over-interpretation of a trend that does not seem to be significant. Please remove or justify.
----

RESPONSE:

We agree with this assessment and significantly tone down our interpretations in the edited text.
----

L. 1120: This is way too strong. The trend found by the authors could contribute to the lack of star-formation but additional factors (AGN feedback being just one of them) need to be considered before making such bold claims. Please correct.
----

RESPONSE:

We agree with this assessment and significantly tone down our interpretations. Please also see our responses to some other comments above.
----

Unless I missed it, I don’t think you say how you define central and satellite galaxies. Please state it in the text.
----

RESPONSE:

We are grateful to the referee for catching this. We have defined centrals and satellites in section 3.1.1 (L. 1209-1210). 
----

Fig. 14: It would be informative to have a reference (in the form of e.g. a horizontal line) for the total galaxy population, regardless of the cosmic structure to which it belongs.
----

RESPONSE:

This is an excellent suggestion by the referee and we have implemented this suggestion in every figure showing the median relationship between galactic properties and sigma_fil (Figs. 9, 12, 13, 14).
----

Section 4 (discussion)

I have read with patience this long (> 500 lines) discussion section. I suggest the authors to make an effort in improving the structure of this discussion so that the messages they aim at conveying are more clearly and transparently delivered. The results deserve to be discussed in a concise way, with less repetitions and back-and-forwards.

For the moment I refrain from making detailed line-by-line comments on this section, because I expect many changes after the major comments I have asked the authors to address.
----

RESPONSE:

We have edited and restructured the discussion section, which we believe reads better now.
----

